Efficient iterative linearised solvers for numerical approximations of stochastic Stefan problems

We present iterative solvers to approximate the solution of numerical schemes for stochastic Stefan problems. After briefly talking about the convergence results, we tackle the question of efficient strategies for solving the nonlinear equation associated with this scheme. We explore several approaches, from a standard Newton technique to linearised solvers. The latter offer the advantage of using the same coefficient matrix of the linearised system in each nonlinear iteration, for all time steps, and across all realisations of the Brownian motions. As a consequence, the system can be factorised once and for all. Although the linearised approach has a slower convergence rate, our sensitivity analysis and the use of adaptive tolerance in both deterministic and stochastic cases provide valuable insights for choosing the most effective solver across various scenarii.

==> chapters/ep/plotepdcpuep1.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{axis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0,ymax=30000,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Regularised}
     \addplot[dotted] coordinates {(4,0) (4,30000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0) (8,30000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0) (12,30000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0) (16,30000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0) (20,30000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
\end{axis}
%%%
% \begin{axis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,
%     ymin=0,ymax=15000,ytick=\empty]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%      \addplot[dotted] coordinates {(4,0) (4,15000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0) (8,15000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0) (12,15000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0) (16,15000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0) (20,15000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
% \end{axis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_{\varepsilonep}=1$}
    \label{fig:ctol100ce1}
 \end{figure}
 %
 %
 %
 \begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{semilogyaxis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0.01, ymax=e^12,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Regularised}
      \addplot[dotted] coordinates {(4,0.01) (4,e^12)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0.01) (8,e^12)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0.01) (12,e^12)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0.01) (16,e^12)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0.01) (20,e^12)} node[pos=0.6,above,rotate=90]{$h=0.031$};
\end{semilogyaxis}
%%%
% \begin{semilogyaxis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,ytick=\empty,
%     ymin=0.01, ymax=e^11]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%       \addplot[dotted] coordinates {(4,0.01) (4,e^11)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0.01) (8,e^11)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0.01) (12,e^11)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0.01) (16,e^11)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0.01) (20,e^11)} node[pos=0.6,above,rotate=90]{$h=0.031$};
% \end{semilogyaxis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_\varepsilon=1$}
    \label{fig:enter-label}
 \end{figure}

==> chapters/ep/plotepdcpuep10.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{axis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0,ymax=30000,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Regularised}
     \addplot[dotted] coordinates {(4,0) (4,30000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0) (8,30000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0) (12,30000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0) (16,30000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0) (20,30000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
\end{axis}
%%%
% \begin{axis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,
%     ymin=0,ymax=15000,ytick=\empty]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%      \addplot[dotted] coordinates {(4,0) (4,15000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0) (8,15000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0) (12,15000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0) (16,15000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0) (20,15000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
% \end{axis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_\varepsilonep=10$}
    \label{fig:ctol100c10}
 \end{figure}
 %
 %
 %
 \begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{semilogyaxis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0.01, ymax=e^12,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Regularised}
      \addplot[dotted] coordinates {(4,0.01) (4,e^12)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0.01) (8,e^12)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0.01) (12,e^12)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0.01) (16,e^12)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0.01) (20,e^12)} node[pos=0.6,above,rotate=90]{$h=0.031$};
\end{semilogyaxis}
%%%
% \begin{semilogyaxis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,ytick=\empty,
%     ymin=0.01, ymax=e^11]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%       \addplot[dotted] coordinates {(4,0.01) (4,e^11)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0.01) (8,e^11)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0.01) (12,e^11)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0.01) (16,e^11)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0.01) (20,e^11)} node[pos=0.6,above,rotate=90]{$h=0.031$};
% \end{semilogyaxis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_\varepsilon=10$}
    \label{fig:ctol100ce10log}
 \end{figure}

==> chapters/tab/cpudsc1.tex <==
\begin{table}[h!]
 \resizebox{1.3\textwidth}{!}{
\begin{tabular}{|llllllll|lllll|}
\hline
\multicolumn{8}{|c|}{Deterministic}                                                                                                                                                                                     & \multicolumn{5}{c|}{Stochastic:   100BMs with 25 CPUs}                                                                           \\ \hline
\multicolumn{3}{|c|}{}                                                              & \multicolumn{3}{c|}{\textbf{Avg\_CPU time (Sec)}}                                           & \multicolumn{2}{c|}{\textbf{Ratio}} & \multicolumn{3}{c|}{\textbf{Avg\_CPU time (Sec)}}                                          & \multicolumn{2}{c|}{\textbf{Ratio}} \\ \hline
\multicolumn{1}{|l|}{Sr.} & \multicolumn{1}{l|}{h}     & \multicolumn{1}{l|}{Ndt}   & \multicolumn{1}{l|}{N}        & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}    & N/LR  & \multicolumn{1}{l|}{N}       & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}   & N/LR   \\ \hline
\multicolumn{1}{|l|}{1}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.39}     & \multicolumn{1}{l|}{0.02}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{18.13}  & 7.81  & \multicolumn{1}{l|}{0.13}    & \multicolumn{1}{l|}{0.13}    & \multicolumn{1}{l|}{0.12}    & \multicolumn{1}{l|}{1.01}  & 1.11   \\ \hline
\multicolumn{1}{|l|}{2}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.12}     & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{2.48}   & 2.56  & \multicolumn{1}{l|}{0.25}    & \multicolumn{1}{l|}{0.21}    & \multicolumn{1}{l|}{0.21}    & \multicolumn{1}{l|}{1.21}  & 1.2    \\ \hline
\multicolumn{1}{|l|}{3}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{0.80}     & \multicolumn{1}{l|}{0.42}    & \multicolumn{1}{l|}{0.39}    & \multicolumn{1}{l|}{1.91}   & 2.02  & \multicolumn{1}{l|}{1.60}    & \multicolumn{1}{l|}{1.18}    & \multicolumn{1}{l|}{1.15}    & \multicolumn{1}{l|}{1.36}  & 1.39   \\ \hline
\multicolumn{1}{|l|}{4}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{5.25}     & \multicolumn{1}{l|}{4.04}    & \multicolumn{1}{l|}{3.56}    & \multicolumn{1}{l|}{1.3}    & 1.47  & \multicolumn{1}{l|}{13.91}   & \multicolumn{1}{l|}{11.91}   & \multicolumn{1}{l|}{11.04}   & \multicolumn{1}{l|}{1.17}  & 1.26   \\ \hline
\multicolumn{1}{|l|}{5}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.04}     & \multicolumn{1}{l|}{0.02}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{1.53}   & 0.78  & \multicolumn{1}{l|}{0.19}    & \multicolumn{1}{l|}{0.14}    & \multicolumn{1}{l|}{0.13}    & \multicolumn{1}{l|}{1.41}  & 1.46   \\ \hline
\multicolumn{1}{|l|}{6}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.21}     & \multicolumn{1}{l|}{0.16}    & \multicolumn{1}{l|}{0.15}    & \multicolumn{1}{l|}{1.32}   & 1.41  & \multicolumn{1}{l|}{0.72}    & \multicolumn{1}{l|}{0.52}    & \multicolumn{1}{l|}{0.53}    & \multicolumn{1}{l|}{1.36}  & 1.36   \\ \hline
\multicolumn{1}{|l|}{7}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{2.00}     & \multicolumn{1}{l|}{1.53}    & \multicolumn{1}{l|}{1.58}    & \multicolumn{1}{l|}{1.31}   & 1.27  & \multicolumn{1}{l|}{6.41}    & \multicolumn{1}{l|}{4.74}    & \multicolumn{1}{l|}{4.68}    & \multicolumn{1}{l|}{1.35}  & 1.37   \\ \hline
\multicolumn{1}{|l|}{8}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{19.89}    & \multicolumn{1}{l|}{15.47}   & \multicolumn{1}{l|}{15.37}   & \multicolumn{1}{l|}{1.29}   & 1.29  & \multicolumn{1}{l|}{63.51}   & \multicolumn{1}{l|}{39.16}   & \multicolumn{1}{l|}{44.95}   & \multicolumn{1}{l|}{1.62}  & 1.41   \\ \hline
\multicolumn{1}{|l|}{9}   & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.20}     & \multicolumn{1}{l|}{0.09}    & \multicolumn{1}{l|}{0.17}    & \multicolumn{1}{l|}{2.34}   & 1.16  & \multicolumn{1}{l|}{0.75}    & \multicolumn{1}{l|}{0.30}    & \multicolumn{1}{l|}{0.30}    & \multicolumn{1}{l|}{2.54}  & 2.49   \\ \hline
\multicolumn{1}{|l|}{10}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{1.02}     & \multicolumn{1}{l|}{0.62}    & \multicolumn{1}{l|}{0.55}    & \multicolumn{1}{l|}{1.64}   & 1.85  & \multicolumn{1}{l|}{2.79}    & \multicolumn{1}{l|}{1.95}    & \multicolumn{1}{l|}{1.92}    & \multicolumn{1}{l|}{1.43}  & 1.46   \\ \hline
\multicolumn{1}{|l|}{11}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{8.18}     & \multicolumn{1}{l|}{6.02}    & \multicolumn{1}{l|}{6.11}    & \multicolumn{1}{l|}{1.36}   & 1.34  & \multicolumn{1}{l|}{25.76}   & \multicolumn{1}{l|}{16.86}   & \multicolumn{1}{l|}{17.10}   & \multicolumn{1}{l|}{1.53}  & 1.51   \\ \hline
\multicolumn{1}{|l|}{12}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{83.18}    & \multicolumn{1}{l|}{61.35}   & \multicolumn{1}{l|}{53.44}   & \multicolumn{1}{l|}{1.36}   & 1.56  & \multicolumn{1}{l|}{254.17}  & \multicolumn{1}{l|}{169.66}  & \multicolumn{1}{l|}{174.89}  & \multicolumn{1}{l|}{1.5}   & 1.45   \\ \hline
\multicolumn{1}{|l|}{13}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{1.56}     & \multicolumn{1}{l|}{0.37}    & \multicolumn{1}{l|}{0.38}    & \multicolumn{1}{l|}{4.23}   & 4.06  & \multicolumn{1}{l|}{5.54}    & \multicolumn{1}{l|}{1.10}    & \multicolumn{1}{l|}{1.16}    & \multicolumn{1}{l|}{5.03}  & 4.79   \\ \hline
\multicolumn{1}{|l|}{14}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{4.96}     & \multicolumn{1}{l|}{2.60}    & \multicolumn{1}{l|}{2.61}    & \multicolumn{1}{l|}{1.91}   & 1.9   & \multicolumn{1}{l|}{16.22}   & \multicolumn{1}{l|}{6.57}    & \multicolumn{1}{l|}{7.31}    & \multicolumn{1}{l|}{2.47}  & 2.22   \\ \hline
\multicolumn{1}{|l|}{15}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{36.57}    & \multicolumn{1}{l|}{24.79}   & \multicolumn{1}{l|}{23.18}   & \multicolumn{1}{l|}{1.48}   & 1.58  & \multicolumn{1}{l|}{115.25}  & \multicolumn{1}{l|}{66.98}   & \multicolumn{1}{l|}{71.14}   & \multicolumn{1}{l|}{1.72}  & 1.62   \\ \hline
\multicolumn{1}{|l|}{16}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{359.50}   & \multicolumn{1}{l|}{246.24}  & \multicolumn{1}{l|}{236.57}  & \multicolumn{1}{l|}{1.46}   & 1.52  & \multicolumn{1}{l|}{1023.72} & \multicolumn{1}{l|}{626.56}  & \multicolumn{1}{l|}{626.29}  & \multicolumn{1}{l|}{1.63}  & 1.63   \\ \hline
\multicolumn{1}{|l|}{17}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{21.89}    & \multicolumn{1}{l|}{2.58}    & \multicolumn{1}{l|}{2.68}    & \multicolumn{1}{l|}{8.49}   & 8.18  & \multicolumn{1}{l|}{67.61}   & \multicolumn{1}{l|}{12.15}   & \multicolumn{1}{l|}{12.75}   & \multicolumn{1}{l|}{5.56}  & 5.3    \\ \hline
\multicolumn{1}{|l|}{18}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{49.40}    & \multicolumn{1}{l|}{11.30}   & \multicolumn{1}{l|}{10.59}   & \multicolumn{1}{l|}{4.37}   & 4.67  & \multicolumn{1}{l|}{163.52}  & \multicolumn{1}{l|}{30.52}   & \multicolumn{1}{l|}{30.96}   & \multicolumn{1}{l|}{5.36}  & 5.28   \\ \hline
\multicolumn{1}{|l|}{19}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{241.67}   & \multicolumn{1}{l|}{99.93}   & \multicolumn{1}{l|}{97.12}   & \multicolumn{1}{l|}{2.42}   & 2.49  & \multicolumn{1}{l|}{709.13}  & \multicolumn{1}{l|}{259.55}  & \multicolumn{1}{l|}{260.69}  & \multicolumn{1}{l|}{2.73}  & 2.72   \\ \hline
\multicolumn{1}{|l|}{20}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{2101.19}  & \multicolumn{1}{l|}{1001.94} & \multicolumn{1}{l|}{1023.01} & \multicolumn{1}{l|}{2.1}    & 2.05  & \multicolumn{1}{l|}{6090.00} & \multicolumn{1}{l|}{2581.71} & \multicolumn{1}{l|}{2598.74} & \multicolumn{1}{l|}{2.36}  & 2.34   \\ \hline
\multicolumn{1}{|l|}{21}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{498.98}   & \multicolumn{1}{l|}{35.88}   & \multicolumn{1}{l|}{35.21}   & \multicolumn{1}{l|}{13.91}  & 14.2  & \multicolumn{1}{l|}{1529.96} & \multicolumn{1}{l|}{209.51}  & \multicolumn{1}{l|}{198.24}  & \multicolumn{1}{l|}{7.3}   & 7.72   \\ \hline
\multicolumn{1}{|l|}{22}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{1508.54}  & \multicolumn{1}{l|}{60.92}   & \multicolumn{1}{l|}{58.42}   & \multicolumn{1}{l|}{24.76}  & 25.8  & \multicolumn{1}{l|}{4798.23} & \multicolumn{1}{l|}{216.18}  & \multicolumn{1}{l|}{208.23}  & \multicolumn{1}{l|}{22.2}  & 23.04  \\ \hline
\multicolumn{1}{|l|}{23}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{3008.54}  & \multicolumn{1}{l|}{404.33}  & \multicolumn{1}{l|}{395.02}  & \multicolumn{1}{l|}{7.44}   & 7.62  & \multicolumn{1}{l|}{9208.41} & \multicolumn{1}{l|}{1128.48} & \multicolumn{1}{l|}{1149.67} & \multicolumn{1}{l|}{8.16}  & 8.01   \\ \hline
\multicolumn{1}{|l|}{24}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{18912.03} & \multicolumn{1}{l|}{4098.62} & \multicolumn{1}{l|}{3722.32} & \multicolumn{1}{l|}{4.61}   & 5.08  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}      &        \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=1$}
\label{tab:cpuc1}
\end{table}

==> chapters/tab/cpudsc10.tex <==
\begin{table}[]
 \resizebox{1.2\textwidth}{!}{
\begin{tabular}{|llllllll|lllll|}
\hline
\multicolumn{8}{|c|}{Deterministic}                                                                                                                                                                                     & \multicolumn{5}{c|}{Stochastic:   100BM with 25 CPUs}                                                                            \\ \hline
\multicolumn{1}{|l|}{}    & \multicolumn{2}{l|}{\textbf{}}                          & \multicolumn{3}{l|}{\textbf{Avg\_CPU time}}                                                 & \multicolumn{2}{l|}{\textbf{Ratio}} & \multicolumn{3}{l|}{\textbf{Avg\_CPU time}}                                                & \multicolumn{2}{l|}{\textbf{Ratio}} \\ \hline
\multicolumn{1}{|l|}{Sr.} & \multicolumn{1}{l|}{h}     & \multicolumn{1}{l|}{Ndt}   & \multicolumn{1}{l|}{N}        & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}    & N/LR  & \multicolumn{1}{l|}{N}       & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}    & N/LR  \\ \hline
\multicolumn{1}{|l|}{1}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.37}     & \multicolumn{1}{l|}{0.02}    & \multicolumn{1}{l|}{0.08}    & \multicolumn{1}{l|}{16.57}  & 4.63  & \multicolumn{1}{l|}{0.16}    & \multicolumn{1}{l|}{0.17}    & \multicolumn{1}{l|}{0.17}    & \multicolumn{1}{l|}{0.94}   & 0.96  \\ \hline
\multicolumn{1}{|l|}{2}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.17}     & \multicolumn{1}{l|}{0.07}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{2.57}   & 3.29  & \multicolumn{1}{l|}{0.33}    & \multicolumn{1}{l|}{0.28}    & \multicolumn{1}{l|}{0.28}    & \multicolumn{1}{l|}{1.19}   & 1.21  \\ \hline
\multicolumn{1}{|l|}{3}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{1.07}     & \multicolumn{1}{l|}{0.72}    & \multicolumn{1}{l|}{0.47}    & \multicolumn{1}{l|}{1.49}   & 2.3   & \multicolumn{1}{l|}{1.82}    & \multicolumn{1}{l|}{1.16}    & \multicolumn{1}{l|}{1.20}    & \multicolumn{1}{l|}{1.58}   & 1.52  \\ \hline
\multicolumn{1}{|l|}{4}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{5.58}     & \multicolumn{1}{l|}{4.02}    & \multicolumn{1}{l|}{3.95}    & \multicolumn{1}{l|}{1.39}   & 1.41  & \multicolumn{1}{l|}{16.05}   & \multicolumn{1}{l|}{10.49}   & \multicolumn{1}{l|}{10.71}   & \multicolumn{1}{l|}{1.53}   & 1.5   \\ \hline
\multicolumn{1}{|l|}{5}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.04}     & \multicolumn{1}{l|}{0.03}    & \multicolumn{1}{l|}{0.03}    & \multicolumn{1}{l|}{1.33}   & 1.4   & \multicolumn{1}{l|}{0.25}    & \multicolumn{1}{l|}{0.20}    & \multicolumn{1}{l|}{0.20}    & \multicolumn{1}{l|}{1.27}   & 1.25  \\ \hline
\multicolumn{1}{|l|}{6}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.33}     & \multicolumn{1}{l|}{0.19}    & \multicolumn{1}{l|}{0.18}    & \multicolumn{1}{l|}{1.8}    & 1.89  & \multicolumn{1}{l|}{0.84}    & \multicolumn{1}{l|}{0.62}    & \multicolumn{1}{l|}{0.64}    & \multicolumn{1}{l|}{1.34}   & 1.3   \\ \hline
\multicolumn{1}{|l|}{7}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{2.13}     & \multicolumn{1}{l|}{1.68}    & \multicolumn{1}{l|}{1.67}    & \multicolumn{1}{l|}{1.27}   & 1.28  & \multicolumn{1}{l|}{6.26}    & \multicolumn{1}{l|}{4.63}    & \multicolumn{1}{l|}{4.62}    & \multicolumn{1}{l|}{1.35}   & 1.36  \\ \hline
\multicolumn{1}{|l|}{8}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{21.53}    & \multicolumn{1}{l|}{16.70}   & \multicolumn{1}{l|}{16.52}   & \multicolumn{1}{l|}{1.29}   & 1.3   & \multicolumn{1}{l|}{60.77}   & \multicolumn{1}{l|}{43.42}   & \multicolumn{1}{l|}{43.32}   & \multicolumn{1}{l|}{1.4}    & 1.4   \\ \hline
\multicolumn{1}{|l|}{9}   & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.22}     & \multicolumn{1}{l|}{0.11}    & \multicolumn{1}{l|}{0.11}    & \multicolumn{1}{l|}{2.02}   & 1.96  & \multicolumn{1}{l|}{0.90}    & \multicolumn{1}{l|}{0.41}    & \multicolumn{1}{l|}{0.43}    & \multicolumn{1}{l|}{2.17}   & 2.07  \\ \hline
\multicolumn{1}{|l|}{10}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{1.09}     & \multicolumn{1}{l|}{0.73}    & \multicolumn{1}{l|}{0.72}    & \multicolumn{1}{l|}{1.5}    & 1.51  & \multicolumn{1}{l|}{3.45}    & \multicolumn{1}{l|}{2.09}    & \multicolumn{1}{l|}{2.11}    & \multicolumn{1}{l|}{1.65}   & 1.64  \\ \hline
\multicolumn{1}{|l|}{11}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{8.89}     & \multicolumn{1}{l|}{6.30}    & \multicolumn{1}{l|}{6.44}    & \multicolumn{1}{l|}{1.41}   & 1.38  & \multicolumn{1}{l|}{26.87}   & \multicolumn{1}{l|}{16.83}   & \multicolumn{1}{l|}{16.89}   & \multicolumn{1}{l|}{1.6}    & 1.59  \\ \hline
\multicolumn{1}{|l|}{12}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{87.22}    & \multicolumn{1}{l|}{62.09}   & \multicolumn{1}{l|}{61.82}   & \multicolumn{1}{l|}{1.4}    & 1.41  & \multicolumn{1}{l|}{250.75}  & \multicolumn{1}{l|}{155.76}  & \multicolumn{1}{l|}{156.18}  & \multicolumn{1}{l|}{1.61}   & 1.61  \\ \hline
\multicolumn{1}{|l|}{13}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{1.69}     & \multicolumn{1}{l|}{0.60}    & \multicolumn{1}{l|}{0.59}    & \multicolumn{1}{l|}{2.83}   & 2.89  & \multicolumn{1}{l|}{7.10}    & \multicolumn{1}{l|}{2.02}    & \multicolumn{1}{l|}{1.91}    & \multicolumn{1}{l|}{3.52}   & 3.72  \\ \hline
\multicolumn{1}{|l|}{14}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{6.07}     & \multicolumn{1}{l|}{3.53}    & \multicolumn{1}{l|}{3.50}    & \multicolumn{1}{l|}{1.72}   & 1.73  & \multicolumn{1}{l|}{22.34}   & \multicolumn{1}{l|}{10.40}   & \multicolumn{1}{l|}{10.34}   & \multicolumn{1}{l|}{2.15}   & 2.16  \\ \hline
\multicolumn{1}{|l|}{15}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{39.51}    & \multicolumn{1}{l|}{25.98}   & \multicolumn{1}{l|}{26.17}   & \multicolumn{1}{l|}{1.52}   & 1.51  & \multicolumn{1}{l|}{128.04}  & \multicolumn{1}{l|}{68.50}   & \multicolumn{1}{l|}{68.29}   & \multicolumn{1}{l|}{1.87}   & 1.87  \\ \hline
\multicolumn{1}{|l|}{16}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{366.07}   & \multicolumn{1}{l|}{246.23}  & \multicolumn{1}{l|}{247.24}  & \multicolumn{1}{l|}{1.49}   & 1.48  & \multicolumn{1}{l|}{1139.92} & \multicolumn{1}{l|}{619.52}  & \multicolumn{1}{l|}{621.66}  & \multicolumn{1}{l|}{1.84}   & 1.83  \\ \hline
\multicolumn{1}{|l|}{17}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{22.19}    & \multicolumn{1}{l|}{9.26}    & \multicolumn{1}{l|}{7.21}    & \multicolumn{1}{l|}{2.4}    & 3.08  & \multicolumn{1}{l|}{97.58}   & \multicolumn{1}{l|}{38.89}   & \multicolumn{1}{l|}{36.66}   & \multicolumn{1}{l|}{2.51}   & 2.66  \\ \hline
\multicolumn{1}{|l|}{18}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{81.25}    & \multicolumn{1}{l|}{34.40}   & \multicolumn{1}{l|}{32.05}   & \multicolumn{1}{l|}{2.36}   & 2.54  & \multicolumn{1}{l|}{357.71}  & \multicolumn{1}{l|}{120.32}  & \multicolumn{1}{l|}{120.43}  & \multicolumn{1}{l|}{2.97}   & 2.97  \\ \hline
\multicolumn{1}{|l|}{19}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{263.10}   & \multicolumn{1}{l|}{137.67}  & \multicolumn{1}{l|}{134.59}  & \multicolumn{1}{l|}{1.91}   & 1.95  & \multicolumn{1}{l|}{1001.47} & \multicolumn{1}{l|}{387.10}  & \multicolumn{1}{l|}{386.57}  & \multicolumn{1}{l|}{2.59}   & 2.59  \\ \hline
\multicolumn{1}{|l|}{20}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{2152.94}  & \multicolumn{1}{l|}{1048.05} & \multicolumn{1}{l|}{1027.84} & \multicolumn{1}{l|}{2.05}   & 2.09  & \multicolumn{1}{l|}{7378.79} & \multicolumn{1}{l|}{2649.68} & \multicolumn{1}{l|}{2613.24} & \multicolumn{1}{l|}{2.78}   & 2.82  \\ \hline
\multicolumn{1}{|l|}{21}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{475.62}   & \multicolumn{1}{l|}{148.87}  & \multicolumn{1}{l|}{127.13}  & \multicolumn{1}{l|}{3.19}   & 3.74  & \multicolumn{1}{l|}{2242.91} & \multicolumn{1}{l|}{696.64}  & \multicolumn{1}{l|}{665.81}  & \multicolumn{1}{l|}{3.22}   & 3.37  \\ \hline
\multicolumn{1}{|l|}{22}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{2060.96}  & \multicolumn{1}{l|}{364.86}  & \multicolumn{1}{l|}{318.92}  & \multicolumn{1}{l|}{5.65}   & 6.46  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       &       \\ \hline
\multicolumn{1}{|l|}{23}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{3177.94}  & \multicolumn{1}{l|}{1117.35} & \multicolumn{1}{l|}{1031.90} & \multicolumn{1}{l|}{2.84}   & 3.08  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       &       \\ \hline
\multicolumn{1}{|l|}{24}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{20397.86} & \multicolumn{1}{l|}{4871.00} & \multicolumn{1}{l|}{4363.29} & \multicolumn{1}{l|}{4.19}   & 4.67  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       &       \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=10$}
\label{tab:cpuc10}
\end{table}

==> chapters/tab/cpudsc100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
 \resizebox{1.2\textwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Deterministic}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Stochastic:   100BM with 25 CPUs}}                                                                                                                                                                                                                                             \\ \hline
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}                                                                                                                                                            & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                               & \multicolumn{2}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                      & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Sr.}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} h}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Ndt}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}   & {\color[HTML]{333333} N/LR} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}  & {\color[HTML]{333333} N/LR} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.40}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.02}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.08}} & {\color[HTML]{333333} 8.18} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.17}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.16}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.16}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.04}} & {\color[HTML]{333333} 1.03} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.15}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.07}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.16}}  & {\color[HTML]{333333} 3}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.32}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.30}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.28}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.08}} & {\color[HTML]{333333} 1.15} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.74}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.73}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.45}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.02}}  & {\color[HTML]{333333} 1.65} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.74}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.39}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.34}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.25}} & {\color[HTML]{333333} 1.29} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.59}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.74}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.74}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.49}}  & {\color[HTML]{333333} 1.49} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 15.59}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10.73}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.88}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.45}} & {\color[HTML]{333333} 1.31} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.03}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.03}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.28}}  & {\color[HTML]{333333} 1.29} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.21}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.22}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.19}} & {\color[HTML]{333333} 1.15} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.33}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.63}}  & {\color[HTML]{333333} 1.72} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.87}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.69}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.67}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.26}} & {\color[HTML]{333333} 1.29} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.16}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.72}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.70}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.25}}  & {\color[HTML]{333333} 1.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.08}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.78}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.87}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.27}} & {\color[HTML]{333333} 1.25} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 8}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21.38}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16.66}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16.68}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.28}}  & {\color[HTML]{333333} 1.28} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 54.17}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 42.69}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 43.04}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.27}} & {\color[HTML]{333333} 1.26} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.22}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.18}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.17}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.26}}  & {\color[HTML]{333333} 1.32} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.83}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.61}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.61}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.37}} & {\color[HTML]{333333} 1.36} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.18}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.89}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.86}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.32}}  & {\color[HTML]{333333} 1.37} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.52}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.72}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.67}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.29}} & {\color[HTML]{333333} 1.32} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9.08}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.78}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.73}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.34}}  & {\color[HTML]{333333} 1.35} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 26.24}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 19.28}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18.63}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.36}} & {\color[HTML]{333333} 1.41} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 12}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 87.63}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 64.03}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 61.65}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.37}}  & {\color[HTML]{333333} 1.42} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 233.37}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 160.52}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 154.09}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.45}} & {\color[HTML]{333333} 1.51} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 13}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.70}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.37}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.21}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.24}}  & {\color[HTML]{333333} 1.41} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.44}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.04}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.28}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.28}} & {\color[HTML]{333333} 1.51} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.45}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.50}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.47}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.17}}  & {\color[HTML]{333333} 1.18} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21.85}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.85}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.11}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.22}} & {\color[HTML]{333333} 1.28} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 15}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 39.72}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 28.34}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 27.17}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.4}}   & {\color[HTML]{333333} 1.46} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 121.94}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 83.52}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 78.52}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.46}} & {\color[HTML]{333333} 1.55} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 358.73}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 236.09}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 234.82}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.52}}  & {\color[HTML]{333333} 1.53} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1053.66}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 621.98}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 634.09}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.69}} & {\color[HTML]{333333} 1.66} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21.30}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 33.97}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 30.36}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.63}}  & {\color[HTML]{333333} 0.7}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 90.66}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 133.55}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 124.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.68}} & {\color[HTML]{333333} 0.73} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 83.09}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 76.80}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 71.40}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.08}}  & {\color[HTML]{333333} 1.16} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 354.44}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 318.66}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 308.46}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.11}} & {\color[HTML]{333333} 1.15} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 19}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 264.62}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 219.21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 210.24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.21}}  & {\color[HTML]{333333} 1.26} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1005.91}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 760.39}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 740.12}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.32}} & {\color[HTML]{333333} 1.36} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2084.36}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1058.78}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1055.92}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.97}}  & {\color[HTML]{333333} 1.97} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7487.08}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2976.95}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2954.91}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.52}} & {\color[HTML]{333333} 2.53} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 442.75}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 606.36}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 553.17}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.73}}  & {\color[HTML]{333333} 0.8}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2151.30}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2640.92}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2464.39}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.81}} & {\color[HTML]{333333} 0.87} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 22}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2072.24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1091.98}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 941.32}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.9}}   & {\color[HTML]{333333} 2.2}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 23}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3217.59}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3306.55}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3090.88}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.97}}  & {\color[HTML]{333333} 1.04} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20372.56}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7154.19}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6572.34}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.85}}  & {\color[HTML]{333333} 3.1}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=100$}
\label{tab:cpu100}
\end{table}

==> chapters/tab/cpudsc1000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
 \resizebox{1.2\textwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Deterministic}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Stochastic:   100BM with 25 CPUs}}                                                                                                                                                                                                                                             \\ \hline
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}                                                                                                                                                            & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                                & \multicolumn{2}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                      & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Sr.}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} h}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Ndt}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}   & {\color[HTML]{333333} N/LR} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}  & {\color[HTML]{333333} N/LR} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.28}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.02}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.07}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.52}} & {\color[HTML]{333333} 4.22} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.98}} & {\color[HTML]{333333} 1}    \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.07}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.09}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.99}}  & {\color[HTML]{333333} 1.42} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.27}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.30}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.24}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.88}} & {\color[HTML]{333333} 1.1}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.92}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.73}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.45}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.25}}  & {\color[HTML]{333333} 2.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.61}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.77}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.31}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.91}} & {\color[HTML]{333333} 1.23} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.69}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.45}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.35}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.36}}  & {\color[HTML]{333333} 1.4}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14.19}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.88}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.36}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.19}} & {\color[HTML]{333333} 1.25} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.01}}  & {\color[HTML]{333333} 0.97} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.02}} & {\color[HTML]{333333} 1.06} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.28}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.41}}  & {\color[HTML]{333333} 1.52} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.78}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.77}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.71}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.02}} & {\color[HTML]{333333} 1.1}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.92}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.65}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.57}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.16}}  & {\color[HTML]{333333} 1.22} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.14}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.89}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.76}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.04}} & {\color[HTML]{333333} 1.29} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 8}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18.18}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14.91}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14.65}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.22}}  & {\color[HTML]{333333} 1.24} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 56.20}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 43.27}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 42.19}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.3}}  & {\color[HTML]{333333} 1.33} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.23}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.24}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.21}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.94}}  & {\color[HTML]{333333} 1.06} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.90}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.99}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.89}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.91}} & {\color[HTML]{333333} 1}    \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.93}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.90}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.12}}  & {\color[HTML]{333333} 1.16} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.42}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.25}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.05}} & {\color[HTML]{333333} 1.07} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7.97}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.77}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.77}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.18}}  & {\color[HTML]{333333} 1.38} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 24.34}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20.36}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.99}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.2}}  & {\color[HTML]{333333} 1.35} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 12}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 75.04}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 56.82}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 55.47}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.32}}  & {\color[HTML]{333333} 1.35} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 233.26}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 171.11}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 167.15}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.36}} & {\color[HTML]{333333} 1.4}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 13}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.51}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.10}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.72}}  & {\color[HTML]{333333} 0.72} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.81}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10.09}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9.88}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.58}} & {\color[HTML]{333333} 0.59} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.71}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7.57}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7.33}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.75}}  & {\color[HTML]{333333} 0.78} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20.50}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 30.83}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 29.20}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.67}} & {\color[HTML]{333333} 0.7}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 15}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 36.29}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 33.43}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 28.58}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.09}}  & {\color[HTML]{333333} 1.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 127.36}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 123.34}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100.83}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.03}} & {\color[HTML]{333333} 1.26} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 321.16}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 226.06}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 216.37}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.42}}  & {\color[HTML]{333333} 1.48} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1101.95}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 757.75}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 714.02}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.45}} & {\color[HTML]{333333} 1.54} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18.51}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 73.84}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 73.28}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & {\color[HTML]{333333} 0.25} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 74.37}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 356.55}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 346.35}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.21}} & {\color[HTML]{333333} 0.21} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 73.33}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 137.54}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 132.00}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.53}}  & {\color[HTML]{333333} 0.56} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 298.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 700.21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 669.23}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.43}} & {\color[HTML]{333333} 0.45} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 19}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 242.77}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 406.06}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 316.71}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.6}}   & {\color[HTML]{333333} 0.77} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 936.66}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1878.95}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1436.36}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.5}}  & {\color[HTML]{333333} 0.65} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1860.42}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1247.13}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1073.16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.49}}  & {\color[HTML]{333333} 1.73} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6954.82}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4844.50}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3918.02}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.44}} & {\color[HTML]{333333} 1.78} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 398.70}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1513.53}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1462.51}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.26}}  & {\color[HTML]{333333} 0.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 22}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1909.59}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2236.54}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2082.46}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.85}}  & {\color[HTML]{333333} 0.92} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 23}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2979.91}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7119.43}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6511.14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.42}}  & {\color[HTML]{333333} 0.46} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18378.39}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 12345.17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9885.04}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.49}}  & {\color[HTML]{333333} 1.86} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=1000$}
\label{tab:cpuc1000}
\end{table}

==> ep/eperplot.tex <==
\begin{figure}\centering  
      \begin{minipage}{0.5\textwidth}
      \ref{epmesh1to3}
      \vspace{0.10cm}
      \end{minipage}  
    \begin{tikzpicture}[scale=0.7]
      \begin{loglogaxis}[
      ymin=0.001, ymax=0.3,
      name=plot1, ytick pos=left,
      legend columns=6, legend to name=epmesh1to3,
      ylabel={$h=0.25$},xlabel={$\delta t=0.1$}
      ]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0625dt0.1.dat};
        \addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L] {ep/eph.0625dt0.1.dat};
        \addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0625dt0.1.dat};
        \addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0625dt0.1.dat};
        \addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0625dt0.1.dat};
       \addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0625dt0.1.dat};
       \addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
        \end{loglogaxis}  
        \hskip 25pt
       \begin{loglogaxis} [ymin=0.001, ymax=0.3,name=plot2,at={(plot1.south east)},xlabel={$\delta t=0.01$}
      ]%,legend columns=3, legend to name=m1n100dmin,legend style={font=\scriptsize}]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0625dt0.01.dat};
        %\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L]  {ep/eph.0625dt0.01.dat};
       % \addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0625dt0.01.dat};
       % \addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0625dt0.01.dat};
        %\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0625dt0.01.dat};
        %\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0625dt0.01.dat};
        %\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
      \end{loglogaxis}
%2nd row
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.7]
      \begin{loglogaxis} [
      ymin=0.001, ymax=0.3,
      name=plot1, ytick pos=left,
      legend columns=6, 
      ylabel={$h=0.0313$},xlabel={$\delta t=0.1$}
      ]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0313dt0.1.dat};
        %\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L] {ep/eph.0313dt0.1.dat};
        %\addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0313dt0.1.dat};
        %\addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0313dt0.1.dat};
        %\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0313dt0.1.dat};
       %\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0313dt0.1.dat};
       %\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
        \end{loglogaxis}  
        \hskip 25pt
       \begin{loglogaxis} [ymin=0.001, ymax=0.3,name=plot2,at={(plot1.south east)},xlabel={$\delta t=0.01$}
      ]%,legend columns=3, legend to name=m1n100dmin,legend style={font=\scriptsize}]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0313dt0.01.dat};
        %%\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L]  {ep/eph.0313dt0.01.dat};
       % %\addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0313dt0.01.dat};
       % %\addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0313dt0.01.dat};
        %%\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0313dt0.01.dat};
        %%\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0313dt0.01.dat};
        %%\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
      \end{loglogaxis}
    \end{tikzpicture}
%3rd row
    \begin{tikzpicture}[scale=0.7]
      \begin{loglogaxis} [
      ymin=0.001, ymax=0.3,
      name=plot1, ytick pos=left,
      legend columns=6, 
      ylabel={$h=0.0156$},xlabel={$\delta t=0.1$}
      ]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0156dt0.1.dat};
        %\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L] {ep/eph.0156dt0.1.dat};
        %\addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0156dt0.1.dat};
        %\addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0156dt0.1.dat};
        %\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0156dt0.1.dat};
       %\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0156dt0.1.dat};
       %\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
        \end{loglogaxis}  
        \hskip 25pt
       \begin{loglogaxis} [ymin=0.001, ymax=0.3,name=plot2,at={(plot1.south east)},xlabel={$\delta t=0.01$}
      ]%,legend columns=3, legend to name=m1n100dmin,legend style={font=\scriptsize}]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0156dt0.01.dat};
        %%\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L]  {ep/eph.0156dt0.01.dat};
       % %\addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0156dt0.01.dat};
       % %\addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0156dt0.01.dat};
        %%\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0156dt0.01.dat};
        %%\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0156dt0.01.dat};
        %%\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
      \end{loglogaxis}
    \end{tikzpicture}
%4th row
    \begin{tikzpicture}[scale=0.7]
      \begin{loglogaxis} [
      ymin=0.001, ymax=0.3,
      name=plot1, ytick pos=left,
      legend columns=6,
      ylabel={$h=0.0078$},xlabel={$\delta t=0.1$}
      ]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0078dt0.1.dat};
        %\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L] {ep/eph.0078dt0.1.dat};
        %\addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0078dt0.1.dat};
        %\addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0078dt0.1.dat};
        %\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0078dt0.1.dat};
       %\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0078dt0.1.dat};
       %\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
        \end{loglogaxis}  
        \hskip 25pt
       \begin{loglogaxis} [ymin=0.001, ymax=0.3,name=plot2,at={(plot1.south east)},xlabel={$\delta t=0.01$}
      ]%,legend columns=3, legend to name=m1n100dmin,legend style={font=\scriptsize}]
        \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan,dashed] table[x=C,y=L2z_N] {ep/eph.0078dt0.01.dat};
        %%\addlegendentry{$E^{N}_{\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta,dashed] table[x=C,y=L2z_L]  {ep/eph.0078dt0.01.dat};
       % %\addlegendentry{$E^{L}_{\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal,dashed] table[x=C,y=L2z_R] {ep/eph.0078dt0.01.dat};
       % %\addlegendentry{$E^{R}_{\zeta(u)}$}
          \addplot [mark=asterisk, mark options={solid,color=cyan}, cyan] table[x=C,y=H1z_N] {ep/eph.0078dt0.01.dat};
        %%\addlegendentry{$E^{N}_{\nabla\zeta(u)}$}
        \addplot [mark=o, mark options={solid,color=magenta}, magenta] table[x=C,y=H1z_L] {ep/eph.0078dt0.01.dat};
        %%\addlegendentry{$E^{L}_{\nabla\zeta(u)}$}
        \addplot [mark=diamond, mark options={solid,color=teal}, teal] table[x=C,y=H1z_R] {ep/eph.0078dt0.01.dat};
        %%\addlegendentry{$E^{R}_{\nabla\zeta(u)}$}
      \end{loglogaxis}
    \end{tikzpicture}
    %\subcaption{Discrete error norms verses $C$}
 % \end{minipage}
  \caption{ Relative errors (on $y$-axis) for $\zeta(u)$ with respect to exact solution in $L^2$ (above) and $H_1$ (below) norms with Newton, Linearised and regularised solvers vs $C_{\varepsilon}$ ( on $x$-axis)}
\label{fig:ep_mesh1_5}
\end{figure}

==> ep/plotepdcpuep1.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{axis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0,ymax=30000,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Regularised}
     \addplot[dotted] coordinates {(4,0) (4,30000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0) (8,30000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0) (12,30000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0) (16,30000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0) (20,30000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
\end{axis}
%%%
% \begin{axis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,
%     ymin=0,ymax=15000,ytick=\empty]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%      \addplot[dotted] coordinates {(4,0) (4,15000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0) (8,15000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0) (12,15000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0) (16,15000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0) (20,15000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
% \end{axis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_{\varepsilonep}=1$}
    \label{fig:ctol100ce1}
 \end{figure}
 %
 %
 %
 \begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{semilogyaxis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0.01, ymax=e^12,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep1.dat};
   \addlegendentry{Regularised}
      \addplot[dotted] coordinates {(4,0.01) (4,e^12)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0.01) (8,e^12)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0.01) (12,e^12)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0.01) (16,e^12)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0.01) (20,e^12)} node[pos=0.6,above,rotate=90]{$h=0.031$};
\end{semilogyaxis}
%%%
% \begin{semilogyaxis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,ytick=\empty,
%     ymin=0.01, ymax=e^11]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%       \addplot[dotted] coordinates {(4,0.01) (4,e^11)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0.01) (8,e^11)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0.01) (12,e^11)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0.01) (16,e^11)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0.01) (20,e^11)} node[pos=0.6,above,rotate=90]{$h=0.031$};
% \end{semilogyaxis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_\varepsilon=1$}
    \label{fig:enter-label}
 \end{figure}

==> ep/plotepdcpuep10.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{axis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0,ymax=30000,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Regularised}
     \addplot[dotted] coordinates {(4,0) (4,30000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0) (8,30000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0) (12,30000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0) (16,30000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0) (20,30000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
\end{axis}
%%%
% \begin{axis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,
%     ymin=0,ymax=15000,ytick=\empty]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%      \addplot[dotted] coordinates {(4,0) (4,15000)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0) (8,15000)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0) (12,15000)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0) (16,15000)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0) (20,15000)} node[pos=0.9,above,rotate=90]{$h=0.031$};
% \end{axis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_\varepsilonep=10$}
    \label{fig:ctol100c10}
 \end{figure}
 %
 %
 %
 \begin{figure}
    \centering
\begin{tikzpicture}[scale=0.6]
\pgfplotsset{
    every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south
    },
}
\begin{semilogyaxis}[name=cpuC100d,legend columns=3,width=12cm,
    tick align=outside,tick pos=lower,
    minor tick style={draw=none},
    extra x ticks={},
    extra x tick style={draw,grid style={draw=none},x tick style={draw},
        xticklabel=\pgfmathprintnumber\tick,
        xticklabel style={rotate=30}},
    axis x line=bottom,axis y line=left,    
    xmin=1,xmax=25,xlabel=Sr No:,
    ymin=0.01, ymax=e^12,ylabel=Cumulative frequency]
    % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
    %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
    % }]
  \addplot[red,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=NCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Newton}
    \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
   table[x=sr, y=LCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Linearised}
     \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
   table[x=sr, y=RCCD] {ep/epdcpuep10.dat};
   \addlegendentry{Regularised}
      \addplot[dotted] coordinates {(4,0.01) (4,e^12)} node[pos=0.9,above,rotate=90]{$h=0.25$};
   \addplot[dotted] coordinates {(8,0.01) (8,e^12)} node[pos=0.9,above,rotate=90]{$h=0.125$};
   \addplot[dotted] coordinates {(12,0.01) (12,e^12)} node[pos=0.9,above,rotate=90]{$h=0.063$};
   \addplot[dotted] coordinates {(16,0.01) (16,e^12)} node[pos=0.9,above,rotate=90]{$h=0.05$};
   \addplot[dotted] coordinates {(20,0.01) (20,e^12)} node[pos=0.6,above,rotate=90]{$h=0.031$};
\end{semilogyaxis}
%%%
% \begin{semilogyaxis}[name=cpuC100s,at={(cpuC100d.south east)},legend columns=3,width=12cm,
%     tick align=outside,tick pos=lower,
%     minor tick style={draw=none},
%     extra x ticks={},
%     extra x tick style={draw,grid style={draw=none},x tick style={draw},
%         xticklabel=\pgfmathprintnumber\tick,
%         xticklabel style={rotate=30}},
%     axis x line=bottom,axis y line=left,    
%     xmin=1,xmax=25,xlabel=Sr No:,ytick=\empty,
%     ymin=0.01, ymax=e^11]
%     % table/create on use/NCCS/.style={% cf. https://tex.stackexchange.com/a/198397
%     %     create col/expr={\pgfmathaccuma + \thisrow{NCD}}   
%     % }]
%   \addplot[red,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=NCCS] {dat/CPUC100.dat};
%    \addlegendentry{Newton}
%     \addplot[blue,thick,mark=+,mark options={color=black,solid}] 
%    table[x=sr, y=LCCS] {dat/CPUC100.dat};
%    \addlegendentry{Linearised}
%      \addplot[green!50!black,thick,mark=diamond,mark options={color=black,solid},dotted] 
%    table[x=sr, y=RCCS] {dat/CPUC100.dat};
%    \addlegendentry{Regularised}
%       \addplot[dotted] coordinates {(4,0.01) (4,e^11)} node[pos=0.9,above,rotate=90]{$h=0.25$};
%    \addplot[dotted] coordinates {(8,0.01) (8,e^11)} node[pos=0.9,above,rotate=90]{$h=0.125$};
%    \addplot[dotted] coordinates {(12,0.01) (12,e^11)} node[pos=0.9,above,rotate=90]{$h=0.063$};
%    \addplot[dotted] coordinates {(16,0.01) (16,e^11)} node[pos=0.9,above,rotate=90]{$h=0.05$};
%    \addplot[dotted] coordinates {(20,0.01) (20,e^11)} node[pos=0.6,above,rotate=90]{$h=0.031$};
% \end{semilogyaxis}
\end{tikzpicture}
    \caption{CPU time comparison for $C=100$ (deterministic and stochastic cases) and $C_\varepsilon=10$}
    \label{fig:ctol100ce10log}
 \end{figure}

==> tab/compCPUBMscaling.tex <==
\begin{table}[]
\begin{tabular}{|l|lll|lll|lll|}
\hline
    M4   & \multicolumn{3}{c|}{$N_{\delta t}$=10}                                      & \multicolumn{3}{c|}{$N_{\delta t}$=100}                                       & \multicolumn{3}{c|}{$N_{\delta t}$=1000}                                         \\ \hline
BM     & \multicolumn{1}{l|}{N}     & \multicolumn{1}{l|}{L}      & R     & \multicolumn{1}{l|}{N}      & \multicolumn{1}{l|}{L}      & R      & \multicolumn{1}{l|}{N}       & \multicolumn{1}{l|}{L}       & R       \\ \hline
1   & \multicolumn{1}{l|}{0.9}  & \multicolumn{1}{l|}{1.2}   & 0.5  & \multicolumn{1}{l|}{3.5}   & \multicolumn{1}{l|}{4.3}   & 3.6   & \multicolumn{1}{l|}{22.9}   & \multicolumn{1}{l|}{20.03}   & 19.0   \\ \hline
10  & \multicolumn{1}{l|}{7.0}  & \multicolumn{1}{l|}{10.1}  & 4.4  & \multicolumn{1}{l|}{29.7}  & \multicolumn{1}{l|}{38.6}  & 32.3  & \multicolumn{1}{l|}{205.9}  & \multicolumn{1}{l|}{185.7}  & 178.2  \\ \hline
100 & \multicolumn{1}{l|}{77.99} & \multicolumn{1}{l|}{113.01} & 47.31 & \multicolumn{1}{l|}{310.59} & \multicolumn{1}{l|}{408} & 335.1 & \multicolumn{1}{l|}{2036.8} & \multicolumn{1}{l|}{1783.4} & 1701.4 \\ \hline
\end{tabular}
\caption{Comparison of CPU time across different Brownian motions for methods N, L, and R.}
\label{tab:BM_scaling}
\end{table}

==> tab/cpudsc1.tex <==
\begin{table}[h!]
 \resizebox{1.3\textwidth}{!}{
\begin{tabular}{|llllllll|lllll|}
\hline
\multicolumn{8}{|c|}{Deterministic}                                                                                                                                                                                     & \multicolumn{5}{c|}{Stochastic:   100BMs with 25 CPUs}                                                                           \\ \hline
\multicolumn{3}{|c|}{}                                                              & \multicolumn{3}{c|}{\textbf{Avg\_CPU time (Sec)}}                                           & \multicolumn{2}{c|}{\textbf{Ratio}} & \multicolumn{3}{c|}{\textbf{Avg\_CPU time (Sec)}}                                          & \multicolumn{2}{c|}{\textbf{Ratio}} \\ \hline
\multicolumn{1}{|l|}{Sr.} & \multicolumn{1}{l|}{h}     & \multicolumn{1}{l|}{Ndt}   & \multicolumn{1}{l|}{N}        & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}    & N/LR  & \multicolumn{1}{l|}{N}       & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}   & N/LR   \\ \hline
\multicolumn{1}{|l|}{1}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.39}     & \multicolumn{1}{l|}{0.02}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{18.13}  & 7.81  & \multicolumn{1}{l|}{0.13}    & \multicolumn{1}{l|}{0.13}    & \multicolumn{1}{l|}{0.12}    & \multicolumn{1}{l|}{1.01}  & 1.11   \\ \hline
\multicolumn{1}{|l|}{2}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.12}     & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{2.48}   & 2.56  & \multicolumn{1}{l|}{0.25}    & \multicolumn{1}{l|}{0.21}    & \multicolumn{1}{l|}{0.21}    & \multicolumn{1}{l|}{1.21}  & 1.2    \\ \hline
\multicolumn{1}{|l|}{3}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{0.80}     & \multicolumn{1}{l|}{0.42}    & \multicolumn{1}{l|}{0.39}    & \multicolumn{1}{l|}{1.91}   & 2.02  & \multicolumn{1}{l|}{1.60}    & \multicolumn{1}{l|}{1.18}    & \multicolumn{1}{l|}{1.15}    & \multicolumn{1}{l|}{1.36}  & 1.39   \\ \hline
\multicolumn{1}{|l|}{4}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{5.25}     & \multicolumn{1}{l|}{4.04}    & \multicolumn{1}{l|}{3.56}    & \multicolumn{1}{l|}{1.3}    & 1.47  & \multicolumn{1}{l|}{13.91}   & \multicolumn{1}{l|}{11.91}   & \multicolumn{1}{l|}{11.04}   & \multicolumn{1}{l|}{1.17}  & 1.26   \\ \hline
\multicolumn{1}{|l|}{5}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.04}     & \multicolumn{1}{l|}{0.02}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{1.53}   & 0.78  & \multicolumn{1}{l|}{0.19}    & \multicolumn{1}{l|}{0.14}    & \multicolumn{1}{l|}{0.13}    & \multicolumn{1}{l|}{1.41}  & 1.46   \\ \hline
\multicolumn{1}{|l|}{6}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.21}     & \multicolumn{1}{l|}{0.16}    & \multicolumn{1}{l|}{0.15}    & \multicolumn{1}{l|}{1.32}   & 1.41  & \multicolumn{1}{l|}{0.72}    & \multicolumn{1}{l|}{0.52}    & \multicolumn{1}{l|}{0.53}    & \multicolumn{1}{l|}{1.36}  & 1.36   \\ \hline
\multicolumn{1}{|l|}{7}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{2.00}     & \multicolumn{1}{l|}{1.53}    & \multicolumn{1}{l|}{1.58}    & \multicolumn{1}{l|}{1.31}   & 1.27  & \multicolumn{1}{l|}{6.41}    & \multicolumn{1}{l|}{4.74}    & \multicolumn{1}{l|}{4.68}    & \multicolumn{1}{l|}{1.35}  & 1.37   \\ \hline
\multicolumn{1}{|l|}{8}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{19.89}    & \multicolumn{1}{l|}{15.47}   & \multicolumn{1}{l|}{15.37}   & \multicolumn{1}{l|}{1.29}   & 1.29  & \multicolumn{1}{l|}{63.51}   & \multicolumn{1}{l|}{39.16}   & \multicolumn{1}{l|}{44.95}   & \multicolumn{1}{l|}{1.62}  & 1.41   \\ \hline
\multicolumn{1}{|l|}{9}   & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.20}     & \multicolumn{1}{l|}{0.09}    & \multicolumn{1}{l|}{0.17}    & \multicolumn{1}{l|}{2.34}   & 1.16  & \multicolumn{1}{l|}{0.75}    & \multicolumn{1}{l|}{0.30}    & \multicolumn{1}{l|}{0.30}    & \multicolumn{1}{l|}{2.54}  & 2.49   \\ \hline
\multicolumn{1}{|l|}{10}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{1.02}     & \multicolumn{1}{l|}{0.62}    & \multicolumn{1}{l|}{0.55}    & \multicolumn{1}{l|}{1.64}   & 1.85  & \multicolumn{1}{l|}{2.79}    & \multicolumn{1}{l|}{1.95}    & \multicolumn{1}{l|}{1.92}    & \multicolumn{1}{l|}{1.43}  & 1.46   \\ \hline
\multicolumn{1}{|l|}{11}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{8.18}     & \multicolumn{1}{l|}{6.02}    & \multicolumn{1}{l|}{6.11}    & \multicolumn{1}{l|}{1.36}   & 1.34  & \multicolumn{1}{l|}{25.76}   & \multicolumn{1}{l|}{16.86}   & \multicolumn{1}{l|}{17.10}   & \multicolumn{1}{l|}{1.53}  & 1.51   \\ \hline
\multicolumn{1}{|l|}{12}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{83.18}    & \multicolumn{1}{l|}{61.35}   & \multicolumn{1}{l|}{53.44}   & \multicolumn{1}{l|}{1.36}   & 1.56  & \multicolumn{1}{l|}{254.17}  & \multicolumn{1}{l|}{169.66}  & \multicolumn{1}{l|}{174.89}  & \multicolumn{1}{l|}{1.5}   & 1.45   \\ \hline
\multicolumn{1}{|l|}{13}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{1.56}     & \multicolumn{1}{l|}{0.37}    & \multicolumn{1}{l|}{0.38}    & \multicolumn{1}{l|}{4.23}   & 4.06  & \multicolumn{1}{l|}{5.54}    & \multicolumn{1}{l|}{1.10}    & \multicolumn{1}{l|}{1.16}    & \multicolumn{1}{l|}{5.03}  & 4.79   \\ \hline
\multicolumn{1}{|l|}{14}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{4.96}     & \multicolumn{1}{l|}{2.60}    & \multicolumn{1}{l|}{2.61}    & \multicolumn{1}{l|}{1.91}   & 1.9   & \multicolumn{1}{l|}{16.22}   & \multicolumn{1}{l|}{6.57}    & \multicolumn{1}{l|}{7.31}    & \multicolumn{1}{l|}{2.47}  & 2.22   \\ \hline
\multicolumn{1}{|l|}{15}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{36.57}    & \multicolumn{1}{l|}{24.79}   & \multicolumn{1}{l|}{23.18}   & \multicolumn{1}{l|}{1.48}   & 1.58  & \multicolumn{1}{l|}{115.25}  & \multicolumn{1}{l|}{66.98}   & \multicolumn{1}{l|}{71.14}   & \multicolumn{1}{l|}{1.72}  & 1.62   \\ \hline
\multicolumn{1}{|l|}{16}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{359.50}   & \multicolumn{1}{l|}{246.24}  & \multicolumn{1}{l|}{236.57}  & \multicolumn{1}{l|}{1.46}   & 1.52  & \multicolumn{1}{l|}{1023.72} & \multicolumn{1}{l|}{626.56}  & \multicolumn{1}{l|}{626.29}  & \multicolumn{1}{l|}{1.63}  & 1.63   \\ \hline
\multicolumn{1}{|l|}{17}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{21.89}    & \multicolumn{1}{l|}{2.58}    & \multicolumn{1}{l|}{2.68}    & \multicolumn{1}{l|}{8.49}   & 8.18  & \multicolumn{1}{l|}{67.61}   & \multicolumn{1}{l|}{12.15}   & \multicolumn{1}{l|}{12.75}   & \multicolumn{1}{l|}{5.56}  & 5.3    \\ \hline
\multicolumn{1}{|l|}{18}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{49.40}    & \multicolumn{1}{l|}{11.30}   & \multicolumn{1}{l|}{10.59}   & \multicolumn{1}{l|}{4.37}   & 4.67  & \multicolumn{1}{l|}{163.52}  & \multicolumn{1}{l|}{30.52}   & \multicolumn{1}{l|}{30.96}   & \multicolumn{1}{l|}{5.36}  & 5.28   \\ \hline
\multicolumn{1}{|l|}{19}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{241.67}   & \multicolumn{1}{l|}{99.93}   & \multicolumn{1}{l|}{97.12}   & \multicolumn{1}{l|}{2.42}   & 2.49  & \multicolumn{1}{l|}{709.13}  & \multicolumn{1}{l|}{259.55}  & \multicolumn{1}{l|}{260.69}  & \multicolumn{1}{l|}{2.73}  & 2.72   \\ \hline
\multicolumn{1}{|l|}{20}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{2101.19}  & \multicolumn{1}{l|}{1001.94} & \multicolumn{1}{l|}{1023.01} & \multicolumn{1}{l|}{2.1}    & 2.05  & \multicolumn{1}{l|}{6090.00} & \multicolumn{1}{l|}{2581.71} & \multicolumn{1}{l|}{2598.74} & \multicolumn{1}{l|}{2.36}  & 2.34   \\ \hline
\multicolumn{1}{|l|}{21}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{498.98}   & \multicolumn{1}{l|}{35.88}   & \multicolumn{1}{l|}{35.21}   & \multicolumn{1}{l|}{13.91}  & 14.2  & \multicolumn{1}{l|}{1529.96} & \multicolumn{1}{l|}{209.51}  & \multicolumn{1}{l|}{198.24}  & \multicolumn{1}{l|}{7.3}   & 7.72   \\ \hline
\multicolumn{1}{|l|}{22}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{1508.54}  & \multicolumn{1}{l|}{60.92}   & \multicolumn{1}{l|}{58.42}   & \multicolumn{1}{l|}{24.76}  & 25.8  & \multicolumn{1}{l|}{4798.23} & \multicolumn{1}{l|}{216.18}  & \multicolumn{1}{l|}{208.23}  & \multicolumn{1}{l|}{22.2}  & 23.04  \\ \hline
\multicolumn{1}{|l|}{23}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{3008.54}  & \multicolumn{1}{l|}{404.33}  & \multicolumn{1}{l|}{395.02}  & \multicolumn{1}{l|}{7.44}   & 7.62  & \multicolumn{1}{l|}{9208.41} & \multicolumn{1}{l|}{1128.48} & \multicolumn{1}{l|}{1149.67} & \multicolumn{1}{l|}{8.16}  & 8.01   \\ \hline
\multicolumn{1}{|l|}{24}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{18912.03} & \multicolumn{1}{l|}{4098.62} & \multicolumn{1}{l|}{3722.32} & \multicolumn{1}{l|}{4.61}   & 5.08  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}      &        \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=1$}
\label{tab:cpuc1}
\end{table}

==> tab/cpudsc10.tex <==
\begin{table}[]
 \resizebox{1.2\textwidth}{!}{
\begin{tabular}{|llllllll|lllll|}
\hline
\multicolumn{8}{|c|}{Deterministic}                                                                                                                                                                                     & \multicolumn{5}{c|}{Stochastic:   100BM with 25 CPUs}                                                                            \\ \hline
\multicolumn{1}{|l|}{}    & \multicolumn{2}{l|}{\textbf{}}                          & \multicolumn{3}{l|}{\textbf{Avg\_CPU time}}                                                 & \multicolumn{2}{l|}{\textbf{Ratio}} & \multicolumn{3}{l|}{\textbf{Avg\_CPU time}}                                                & \multicolumn{2}{l|}{\textbf{Ratio}} \\ \hline
\multicolumn{1}{|l|}{Sr.} & \multicolumn{1}{l|}{h}     & \multicolumn{1}{l|}{Ndt}   & \multicolumn{1}{l|}{N}        & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}    & N/LR  & \multicolumn{1}{l|}{N}       & \multicolumn{1}{l|}{L}       & \multicolumn{1}{l|}{LR}      & \multicolumn{1}{l|}{N/L}    & N/LR  \\ \hline
\multicolumn{1}{|l|}{1}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.37}     & \multicolumn{1}{l|}{0.02}    & \multicolumn{1}{l|}{0.08}    & \multicolumn{1}{l|}{16.57}  & 4.63  & \multicolumn{1}{l|}{0.16}    & \multicolumn{1}{l|}{0.17}    & \multicolumn{1}{l|}{0.17}    & \multicolumn{1}{l|}{0.94}   & 0.96  \\ \hline
\multicolumn{1}{|l|}{2}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.17}     & \multicolumn{1}{l|}{0.07}    & \multicolumn{1}{l|}{0.05}    & \multicolumn{1}{l|}{2.57}   & 3.29  & \multicolumn{1}{l|}{0.33}    & \multicolumn{1}{l|}{0.28}    & \multicolumn{1}{l|}{0.28}    & \multicolumn{1}{l|}{1.19}   & 1.21  \\ \hline
\multicolumn{1}{|l|}{3}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{1.07}     & \multicolumn{1}{l|}{0.72}    & \multicolumn{1}{l|}{0.47}    & \multicolumn{1}{l|}{1.49}   & 2.3   & \multicolumn{1}{l|}{1.82}    & \multicolumn{1}{l|}{1.16}    & \multicolumn{1}{l|}{1.20}    & \multicolumn{1}{l|}{1.58}   & 1.52  \\ \hline
\multicolumn{1}{|l|}{4}   & \multicolumn{1}{l|}{0.25}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{5.58}     & \multicolumn{1}{l|}{4.02}    & \multicolumn{1}{l|}{3.95}    & \multicolumn{1}{l|}{1.39}   & 1.41  & \multicolumn{1}{l|}{16.05}   & \multicolumn{1}{l|}{10.49}   & \multicolumn{1}{l|}{10.71}   & \multicolumn{1}{l|}{1.53}   & 1.5   \\ \hline
\multicolumn{1}{|l|}{5}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.04}     & \multicolumn{1}{l|}{0.03}    & \multicolumn{1}{l|}{0.03}    & \multicolumn{1}{l|}{1.33}   & 1.4   & \multicolumn{1}{l|}{0.25}    & \multicolumn{1}{l|}{0.20}    & \multicolumn{1}{l|}{0.20}    & \multicolumn{1}{l|}{1.27}   & 1.25  \\ \hline
\multicolumn{1}{|l|}{6}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{0.33}     & \multicolumn{1}{l|}{0.19}    & \multicolumn{1}{l|}{0.18}    & \multicolumn{1}{l|}{1.8}    & 1.89  & \multicolumn{1}{l|}{0.84}    & \multicolumn{1}{l|}{0.62}    & \multicolumn{1}{l|}{0.64}    & \multicolumn{1}{l|}{1.34}   & 1.3   \\ \hline
\multicolumn{1}{|l|}{7}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{2.13}     & \multicolumn{1}{l|}{1.68}    & \multicolumn{1}{l|}{1.67}    & \multicolumn{1}{l|}{1.27}   & 1.28  & \multicolumn{1}{l|}{6.26}    & \multicolumn{1}{l|}{4.63}    & \multicolumn{1}{l|}{4.62}    & \multicolumn{1}{l|}{1.35}   & 1.36  \\ \hline
\multicolumn{1}{|l|}{8}   & \multicolumn{1}{l|}{0.125} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{21.53}    & \multicolumn{1}{l|}{16.70}   & \multicolumn{1}{l|}{16.52}   & \multicolumn{1}{l|}{1.29}   & 1.3   & \multicolumn{1}{l|}{60.77}   & \multicolumn{1}{l|}{43.42}   & \multicolumn{1}{l|}{43.32}   & \multicolumn{1}{l|}{1.4}    & 1.4   \\ \hline
\multicolumn{1}{|l|}{9}   & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{0.22}     & \multicolumn{1}{l|}{0.11}    & \multicolumn{1}{l|}{0.11}    & \multicolumn{1}{l|}{2.02}   & 1.96  & \multicolumn{1}{l|}{0.90}    & \multicolumn{1}{l|}{0.41}    & \multicolumn{1}{l|}{0.43}    & \multicolumn{1}{l|}{2.17}   & 2.07  \\ \hline
\multicolumn{1}{|l|}{10}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{1.09}     & \multicolumn{1}{l|}{0.73}    & \multicolumn{1}{l|}{0.72}    & \multicolumn{1}{l|}{1.5}    & 1.51  & \multicolumn{1}{l|}{3.45}    & \multicolumn{1}{l|}{2.09}    & \multicolumn{1}{l|}{2.11}    & \multicolumn{1}{l|}{1.65}   & 1.64  \\ \hline
\multicolumn{1}{|l|}{11}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{8.89}     & \multicolumn{1}{l|}{6.30}    & \multicolumn{1}{l|}{6.44}    & \multicolumn{1}{l|}{1.41}   & 1.38  & \multicolumn{1}{l|}{26.87}   & \multicolumn{1}{l|}{16.83}   & \multicolumn{1}{l|}{16.89}   & \multicolumn{1}{l|}{1.6}    & 1.59  \\ \hline
\multicolumn{1}{|l|}{12}  & \multicolumn{1}{l|}{0.063} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{87.22}    & \multicolumn{1}{l|}{62.09}   & \multicolumn{1}{l|}{61.82}   & \multicolumn{1}{l|}{1.4}    & 1.41  & \multicolumn{1}{l|}{250.75}  & \multicolumn{1}{l|}{155.76}  & \multicolumn{1}{l|}{156.18}  & \multicolumn{1}{l|}{1.61}   & 1.61  \\ \hline
\multicolumn{1}{|l|}{13}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{1.69}     & \multicolumn{1}{l|}{0.60}    & \multicolumn{1}{l|}{0.59}    & \multicolumn{1}{l|}{2.83}   & 2.89  & \multicolumn{1}{l|}{7.10}    & \multicolumn{1}{l|}{2.02}    & \multicolumn{1}{l|}{1.91}    & \multicolumn{1}{l|}{3.52}   & 3.72  \\ \hline
\multicolumn{1}{|l|}{14}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{6.07}     & \multicolumn{1}{l|}{3.53}    & \multicolumn{1}{l|}{3.50}    & \multicolumn{1}{l|}{1.72}   & 1.73  & \multicolumn{1}{l|}{22.34}   & \multicolumn{1}{l|}{10.40}   & \multicolumn{1}{l|}{10.34}   & \multicolumn{1}{l|}{2.15}   & 2.16  \\ \hline
\multicolumn{1}{|l|}{15}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{39.51}    & \multicolumn{1}{l|}{25.98}   & \multicolumn{1}{l|}{26.17}   & \multicolumn{1}{l|}{1.52}   & 1.51  & \multicolumn{1}{l|}{128.04}  & \multicolumn{1}{l|}{68.50}   & \multicolumn{1}{l|}{68.29}   & \multicolumn{1}{l|}{1.87}   & 1.87  \\ \hline
\multicolumn{1}{|l|}{16}  & \multicolumn{1}{l|}{0.05}  & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{366.07}   & \multicolumn{1}{l|}{246.23}  & \multicolumn{1}{l|}{247.24}  & \multicolumn{1}{l|}{1.49}   & 1.48  & \multicolumn{1}{l|}{1139.92} & \multicolumn{1}{l|}{619.52}  & \multicolumn{1}{l|}{621.66}  & \multicolumn{1}{l|}{1.84}   & 1.83  \\ \hline
\multicolumn{1}{|l|}{17}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{22.19}    & \multicolumn{1}{l|}{9.26}    & \multicolumn{1}{l|}{7.21}    & \multicolumn{1}{l|}{2.4}    & 3.08  & \multicolumn{1}{l|}{97.58}   & \multicolumn{1}{l|}{38.89}   & \multicolumn{1}{l|}{36.66}   & \multicolumn{1}{l|}{2.51}   & 2.66  \\ \hline
\multicolumn{1}{|l|}{18}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{81.25}    & \multicolumn{1}{l|}{34.40}   & \multicolumn{1}{l|}{32.05}   & \multicolumn{1}{l|}{2.36}   & 2.54  & \multicolumn{1}{l|}{357.71}  & \multicolumn{1}{l|}{120.32}  & \multicolumn{1}{l|}{120.43}  & \multicolumn{1}{l|}{2.97}   & 2.97  \\ \hline
\multicolumn{1}{|l|}{19}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{263.10}   & \multicolumn{1}{l|}{137.67}  & \multicolumn{1}{l|}{134.59}  & \multicolumn{1}{l|}{1.91}   & 1.95  & \multicolumn{1}{l|}{1001.47} & \multicolumn{1}{l|}{387.10}  & \multicolumn{1}{l|}{386.57}  & \multicolumn{1}{l|}{2.59}   & 2.59  \\ \hline
\multicolumn{1}{|l|}{20}  & \multicolumn{1}{l|}{0.031} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{2152.94}  & \multicolumn{1}{l|}{1048.05} & \multicolumn{1}{l|}{1027.84} & \multicolumn{1}{l|}{2.05}   & 2.09  & \multicolumn{1}{l|}{7378.79} & \multicolumn{1}{l|}{2649.68} & \multicolumn{1}{l|}{2613.24} & \multicolumn{1}{l|}{2.78}   & 2.82  \\ \hline
\multicolumn{1}{|l|}{21}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10}    & \multicolumn{1}{l|}{475.62}   & \multicolumn{1}{l|}{148.87}  & \multicolumn{1}{l|}{127.13}  & \multicolumn{1}{l|}{3.19}   & 3.74  & \multicolumn{1}{l|}{2242.91} & \multicolumn{1}{l|}{696.64}  & \multicolumn{1}{l|}{665.81}  & \multicolumn{1}{l|}{3.22}   & 3.37  \\ \hline
\multicolumn{1}{|l|}{22}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{100}   & \multicolumn{1}{l|}{2060.96}  & \multicolumn{1}{l|}{364.86}  & \multicolumn{1}{l|}{318.92}  & \multicolumn{1}{l|}{5.65}   & 6.46  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       &       \\ \hline
\multicolumn{1}{|l|}{23}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{1000}  & \multicolumn{1}{l|}{3177.94}  & \multicolumn{1}{l|}{1117.35} & \multicolumn{1}{l|}{1031.90} & \multicolumn{1}{l|}{2.84}   & 3.08  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       &       \\ \hline
\multicolumn{1}{|l|}{24}  & \multicolumn{1}{l|}{0.008} & \multicolumn{1}{l|}{10000} & \multicolumn{1}{l|}{20397.86} & \multicolumn{1}{l|}{4871.00} & \multicolumn{1}{l|}{4363.29} & \multicolumn{1}{l|}{4.19}   & 4.67  & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       &       \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=10$}
\label{tab:cpuc10}
\end{table}

==> tab/cpudsc100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
 \resizebox{1.2\textwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Deterministic}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Stochastic:   100BM with 25 CPUs}}                                                                                                                                                                                                                                             \\ \hline
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}                                                                                                                                                            & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                               & \multicolumn{2}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                      & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Sr.}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} h}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Ndt}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}   & {\color[HTML]{333333} N/LR} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}  & {\color[HTML]{333333} N/LR} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.40}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.02}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.08}} & {\color[HTML]{333333} 8.18} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.17}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.16}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.16}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.04}} & {\color[HTML]{333333} 1.03} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.15}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.07}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.16}}  & {\color[HTML]{333333} 3}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.32}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.30}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.28}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.08}} & {\color[HTML]{333333} 1.15} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.74}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.73}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.45}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.02}}  & {\color[HTML]{333333} 1.65} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.74}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.39}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.34}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.25}} & {\color[HTML]{333333} 1.29} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.59}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.74}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.74}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.49}}  & {\color[HTML]{333333} 1.49} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 15.59}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10.73}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.88}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.45}} & {\color[HTML]{333333} 1.31} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.03}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.03}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.28}}  & {\color[HTML]{333333} 1.29} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.21}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.22}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.19}} & {\color[HTML]{333333} 1.15} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.33}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.63}}  & {\color[HTML]{333333} 1.72} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.87}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.69}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.67}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.26}} & {\color[HTML]{333333} 1.29} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.16}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.72}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.70}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.25}}  & {\color[HTML]{333333} 1.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.08}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.78}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.87}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.27}} & {\color[HTML]{333333} 1.25} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 8}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21.38}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16.66}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16.68}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.28}}  & {\color[HTML]{333333} 1.28} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 54.17}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 42.69}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 43.04}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.27}} & {\color[HTML]{333333} 1.26} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.22}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.18}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.17}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.26}}  & {\color[HTML]{333333} 1.32} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.83}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.61}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.61}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.37}} & {\color[HTML]{333333} 1.36} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.18}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.89}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.86}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.32}}  & {\color[HTML]{333333} 1.37} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.52}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.72}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.67}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.29}} & {\color[HTML]{333333} 1.32} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9.08}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.78}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.73}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.34}}  & {\color[HTML]{333333} 1.35} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 26.24}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 19.28}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18.63}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.36}} & {\color[HTML]{333333} 1.41} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 12}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 87.63}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 64.03}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 61.65}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.37}}  & {\color[HTML]{333333} 1.42} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 233.37}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 160.52}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 154.09}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.45}} & {\color[HTML]{333333} 1.51} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 13}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.70}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.37}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.21}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.24}}  & {\color[HTML]{333333} 1.41} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.44}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.04}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.28}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.28}} & {\color[HTML]{333333} 1.51} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.45}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.50}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.47}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.17}}  & {\color[HTML]{333333} 1.18} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21.85}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.85}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.11}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.22}} & {\color[HTML]{333333} 1.28} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 15}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 39.72}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 28.34}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 27.17}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.4}}   & {\color[HTML]{333333} 1.46} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 121.94}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 83.52}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 78.52}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.46}} & {\color[HTML]{333333} 1.55} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 358.73}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 236.09}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 234.82}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.52}}  & {\color[HTML]{333333} 1.53} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1053.66}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 621.98}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 634.09}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.69}} & {\color[HTML]{333333} 1.66} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21.30}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 33.97}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 30.36}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.63}}  & {\color[HTML]{333333} 0.7}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 90.66}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 133.55}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 124.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.68}} & {\color[HTML]{333333} 0.73} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 83.09}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 76.80}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 71.40}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.08}}  & {\color[HTML]{333333} 1.16} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 354.44}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 318.66}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 308.46}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.11}} & {\color[HTML]{333333} 1.15} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 19}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 264.62}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 219.21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 210.24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.21}}  & {\color[HTML]{333333} 1.26} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1005.91}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 760.39}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 740.12}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.32}} & {\color[HTML]{333333} 1.36} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2084.36}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1058.78}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1055.92}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.97}}  & {\color[HTML]{333333} 1.97} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7487.08}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2976.95}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2954.91}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.52}} & {\color[HTML]{333333} 2.53} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 442.75}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 606.36}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 553.17}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.73}}  & {\color[HTML]{333333} 0.8}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2151.30}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2640.92}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2464.39}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.81}} & {\color[HTML]{333333} 0.87} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 22}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2072.24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1091.98}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 941.32}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.9}}   & {\color[HTML]{333333} 2.2}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 23}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3217.59}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3306.55}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3090.88}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.97}}  & {\color[HTML]{333333} 1.04} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20372.56}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7154.19}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6572.34}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.85}}  & {\color[HTML]{333333} 3.1}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=100$}
\label{tab:cpu100}
\end{table}

==> tab/cpudsc1000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
 \resizebox{1.2\textwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\multicolumn{8}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Deterministic}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Stochastic:   100BM with 25 CPUs}}                                                                                                                                                                                                                                             \\ \hline
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}                                                                                                                                                            & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                                & \multicolumn{2}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                      & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Avg\_CPU time}}}                                                                                                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Ratio}}}                     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Sr.}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} h}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Ndt}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}   & {\color[HTML]{333333} N/LR} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} L}}       & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} LR}}      & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} N/L}}  & {\color[HTML]{333333} N/LR} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.28}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.02}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.07}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.52}} & {\color[HTML]{333333} 4.22} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.98}} & {\color[HTML]{333333} 1}    \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.13}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.07}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.09}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.99}}  & {\color[HTML]{333333} 1.42} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.27}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.30}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.24}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.88}} & {\color[HTML]{333333} 1.1}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.92}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.73}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.45}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.25}}  & {\color[HTML]{333333} 2.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.61}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.77}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.31}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.91}} & {\color[HTML]{333333} 1.23} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.69}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.45}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.35}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.36}}  & {\color[HTML]{333333} 1.4}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14.19}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.88}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11.36}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.19}} & {\color[HTML]{333333} 1.25} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.04}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.01}}  & {\color[HTML]{333333} 0.97} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.02}} & {\color[HTML]{333333} 1.06} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.28}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.20}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.41}}  & {\color[HTML]{333333} 1.52} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.78}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.77}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.71}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.02}} & {\color[HTML]{333333} 1.1}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.92}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.65}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.57}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.16}}  & {\color[HTML]{333333} 1.22} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.14}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.89}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4.76}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.04}} & {\color[HTML]{333333} 1.29} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 8}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.125}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18.18}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14.91}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14.65}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.22}}  & {\color[HTML]{333333} 1.24} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 56.20}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 43.27}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 42.19}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.3}}  & {\color[HTML]{333333} 1.33} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.23}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.24}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.21}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.94}}  & {\color[HTML]{333333} 1.06} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.90}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.99}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.89}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.91}} & {\color[HTML]{333333} 1}    \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.04}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.93}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.90}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.12}}  & {\color[HTML]{333333} 1.16} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.42}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.25}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3.19}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.05}} & {\color[HTML]{333333} 1.07} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 11}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7.97}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6.77}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.77}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.18}}  & {\color[HTML]{333333} 1.38} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 24.34}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20.36}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17.99}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.2}}  & {\color[HTML]{333333} 1.35} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 12}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.063}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 75.04}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 56.82}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 55.47}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.32}}  & {\color[HTML]{333333} 1.35} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 233.26}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 171.11}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 167.15}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.36}} & {\color[HTML]{333333} 1.4}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 13}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.51}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.10}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2.10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.72}}  & {\color[HTML]{333333} 0.72} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.81}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10.09}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9.88}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.58}} & {\color[HTML]{333333} 0.59} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 14}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 5.71}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7.57}}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7.33}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.75}}  & {\color[HTML]{333333} 0.78} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20.50}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 30.83}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 29.20}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.67}} & {\color[HTML]{333333} 0.7}  \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 15}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 36.29}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 33.43}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 28.58}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.09}}  & {\color[HTML]{333333} 1.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 127.36}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 123.34}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100.83}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.03}} & {\color[HTML]{333333} 1.26} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.05}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 321.16}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 226.06}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 216.37}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.42}}  & {\color[HTML]{333333} 1.48} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1101.95}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 757.75}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 714.02}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.45}} & {\color[HTML]{333333} 1.54} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 17}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18.51}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 73.84}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 73.28}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.25}}  & {\color[HTML]{333333} 0.25} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 74.37}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 356.55}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 346.35}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.21}} & {\color[HTML]{333333} 0.21} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 73.33}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 137.54}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 132.00}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.53}}  & {\color[HTML]{333333} 0.56} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 298.25}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 700.21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 669.23}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.43}} & {\color[HTML]{333333} 0.45} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 19}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 242.77}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 406.06}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 316.71}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.6}}   & {\color[HTML]{333333} 0.77} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 936.66}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1878.95}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1436.36}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.5}}  & {\color[HTML]{333333} 0.65} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 20}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.031}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1860.42}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1247.13}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1073.16}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.49}}  & {\color[HTML]{333333} 1.73} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6954.82}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4844.50}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 3918.02}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.44}} & {\color[HTML]{333333} 1.78} \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 21}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10}}    & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 398.70}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1513.53}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1462.51}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.26}}  & {\color[HTML]{333333} 0.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 22}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 100}}   & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1909.59}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2236.54}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2082.46}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.85}}  & {\color[HTML]{333333} 0.92} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 23}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1000}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 2979.91}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 7119.43}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 6511.14}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.42}}  & {\color[HTML]{333333} 0.46} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 24}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.008}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10000}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 18378.39}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 12345.17}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 9885.04}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.49}}  & {\color[HTML]{333333} 1.86} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}        & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}     & {\color[HTML]{333333} }     \\ \hline
\end{tabular}
}
\caption{CPU time comparison for $C=1000$}
\label{tab:cpuc1000}
\end{table}

==> tab/res_comph0.125dt0.01.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
$C_{tol}$    & $tol$  & res\_N   & res\_L   & res\_R   \\ \hline
1    & 1.25E-01 & 1.61E-03 & 7.11E-03 & 6.91E-03 \\ \hline
10   & 1.25E-02 & 1.16E-04 & 7.59E-04 & 7.44E-04 \\ \hline
100  & 1.25E-03 & 4.04E-17 & 7.99E-05 & 7.91E-05 \\ \hline
1000 & 1.25E-04 & 4.04E-17 & 8.17E-06 & 7.99E-06 \\ \hline
\end{tabular}
\caption{$h=0.125$ and $dt=0.01$}
\label{tab:residue_comp}
\end{table}

==> tab/trimesh.tex <==
\begin{table}%[h!]
										\centering
										\caption{Data for the triangular meshes}%
										\label{tab:tri_mesh}
										\begin{tabular}{|c|c|c|c|c|}
												\hline
												Mesh& Size& Cells & Edges&Vertices\\
												\hline
												M1&    0.250&   56&     92&     37\\%16    
												M2&    0.125&   224&    352&    129\\%64
												M3&    0.0625&   896&    1376&   481\\%256
												M4&    0.0313&   3584&   5440&   1857\\%400
												M5&    0.0156&   14336&   21632&   7297\\%1024
												M6&    0.0078&   57344&  86272&  28929\\%4096
												\hline	
											\end{tabular}%
										%
	\end{table}%
